Propeller Modulation Equalization via Reference Tones

Propeller modulation, also known as micro-Doppler modulation, presents a significant challenge in radio frequency (RF) inspection operations conducted via drones. This paper investigates the equalization of propeller modulation effects on RF signals, specifically targeting applications in navigation aids such as Instrument Landing Systems (ILS). By employing a continuous reference tone, the propeller-induced Doppler spread can be effectively captured and equalized, improving signal integrity and accuracy. Simulation results demonstrate that the proposed equalization method significantly reduces DDM deviation caused by propeller modulation, even under various propeller speeds. The findings suggest that incorporating such equalization techniques can enhance the reliability and efficiency of drone-based RF inspections.

==> draft <==
This paper focuses on equalizing propeller modulation in radio frequency (RF) inspection operations conducted via drones. The future of RF inspections for Federal Aviation Administration (FAA) services, such as Instrument Landing System (ILS) and VHF Omnidirectional Range (VOR) or radar services, is projected to rely on unmanned aerial vehicles (UAVs), which utilize propellers for hovering. These drones can be used for navigation aids (NAVAIDS) inspection, as reported by the International Civil Aviation Organization (ICAO), and several companies already offer this service. Additionally, drones are proposed for radar calibration \cite{boyer2017uav,yin2019uav} and antenna pattern measurements \cite{salazar2023accuracy,garcia2017antenna,segales2023far,culotta2021uncertainty,fernandez2018use,salari2021unmanned}.

Propeller modulation, also known as micro-Doppler propeller modulation, is a channel disruptor caused either by cutting the direct signal path or altering the reflective environment around the receiver attached to the drone. This effect has been characterized in the literature through simulations, measurements, and mathematical models in several studies \cite{marak2017electromagnetic,faul2021impact}. Propeller modulation has also been utilized for drone recognition and classification \cite{mingjiu2022rotor,chen2019signal,ezuma2022comparative,maasdorp2015fm,pan2013modulation,liu2017micro,yong2016research}, and specifically for drones and propeller parameter extraction \cite{kang20206}. However, these studies primarily focus on radar theory and do not address the impairment in communication or inspection systems.

The impairments caused by propeller modulation were reported in the Scanning Beam Microwave Landing System \cite{pope1974propeller}. The Pilot’s Handbook of Aeronautical Knowledge \cite{federal2009pilot} reports that specific propeller RPM settings or helicopter rotor speeds can affect the VOR course deviation indicator. Additionally, certain engine RPM settings in propeller-powered planes can impact the auto-pilot system that relies on ILS measurements \cite{duncanaviation2019propeller}. This aligns with studies on ILS inspection that identify propeller modulation as a measurement noise \cite{horapong2017design,ibrahim2022unmanned,8448050,bredemeyer2018employing}. In ILS, for instance, the propeller causes interference between the center tone and the 90Hz and 150Hz tones.

 This paper investigates the possibility of equalizing the propeller modulation effect for communication purposes and radio frequency inspections. We argue that equalization is more critical for the latter, as modern communications use wide bandwidth bursts, and subcarrier spacing can be adjusted to accommodate Doppler spreads. However, NAVAIDS and radar signals, such as ILS, VOR, and frequency modulated continuous wave (FMCW) chirps, are continuous and require equalization to obtain accurate inspection data. Without equalization, averaging would be necessary to manage the time variation of the channel, resulting in longer inspection times.
 
%Doppler spread equalization in a communication system depends on reference signals, also called pilots, sent along with the data from the same transmitter. 
%In our work, we propose to use the same technique but with the pilots transmitted from another transmitter. This is due to the inflexibility of the inspected system, its old age, and that it was not built in time when drones were used to do measurements.  The proposed setup is shown in the below figure. 


The rest of this paper is organized as follows; 



\section{Simulation and Discussion}
In this section, we evaluate the equalization process assuming the signal under propeller doppler spread is an ILS signal. An ILS signal is ( short brief) composed of a carrier and a $\pm 90~Hz$, and $\pm 150~Hz$ modulations. The side carriers are transmitted over offseted beams to give position information from relative to the carrier amplitudes. The position is calculated from DDM as: 
\begin{equation}
    DDM = \dfrac{A_{90}- A_c}{A_c} - \dfrac{A_{150}- A_c}{A_c}, 
    \label{eq:DDM}
\end{equation}
where $A_c,~A_{90}$and ,$~A_{150}$ are the amplitudes of the carrier, 90 Hz and 150 Hz modulations respectively. 

In the presence of propeller modulation, there is an interference between the components of the ILS signal, and in order to resolve it we transmit the pilot tone 1.5 KHz away from the ILS signal, as shown in Fig. \ref{fig:simmodulated}. The figure shows the modulation effect in frequency domain on the combined signal $ \mathbb{S}(f)+ \mathbb{T}(f)$.

The propeller modulation used in this simulation is formulated as
\begin{equation}
    R(t) =  S(t-\tau_p)~g(2 \pi f_p t),
\end{equation}
and $g$ is a square wave, which gives a harsh modulation effect due to the sinc-shaped frequency domain of it. We capture $\pm 300~Hz$ of the modulated tone and use it to equalize the signal using Eq. (\ref{eq:equalization}). The equalization results are shown in Fig. \ref{fig:simequalized}. We notice that the equalization resulted in a pure reference tone and ILS signal, but it created a noise floor although there is no noise added to the modulation step. But even with this noise floor, the signal performance is better due to the recovered signal integrity. 

The parameters of the simulation are: sampling rate=32KHz, capture duration in time is 1 sec, FFT and IFFT sizes is 32000, hence a one-to-one relationship between the frequency bins and frequency in Hz. The channel as additive white gaussian noise with one tap that is doppler modulated with $g(t)$.  
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig1_modulated.eps}
        \caption{Propeller modulated  $\left( \mathbb{S}(f)+ \mathbb{T}(f) \right)$.}
        \label{fig:simmodulated}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
    \includegraphics[width=\textwidth]{fig1_equalized.eps}
        \caption{Equalized  $\left( \mathbb{S}(f)+ \mathbb{T}(f) \right)$}
        \label{fig:simequalized}
    \end{subfigure}
    \caption{Comparison of Propeller Modulated and Equalized  $\left( \mathbb{S}(f)+ \mathbb{T}(f) \right)$.}
    \label{fig:comparison}
\end{figure}

We evaluate the signal integrity through calculating the DDM error before and after equalization. The transmitted tone amplitudes are $A_c=1 v, A_{90}=0.6 v, and A_{150}=0.8 v$, assuming the amplitude unit is in 
volts. The DDM value is -0.2  and it is unitless. For a realistic scenario we assume SNR of 20 dB. The received DDM drift is calculated for different $f_p$ values, emulating different propeller speeds, and shown in Fig. \ref{fig:speed}. The range of $f_p$ is [15, 40] Hz.  Which passes through points where the interference between the ILS tones is at its highest point, we can observe this at $f_p~=17,~20,~26,~30, ~and ~36 Hz$. Note that the modulating signal we chose is only for demonstration and it will change from drone to drone and with set of propeller movements and speeds. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{prelimspeedresults2.pdf}
    \caption{Prelim speed results.}
    \label{fig:speed}
\end{figure*}
We can see that the equalized signal DDM deviation is much lower the nonequalized signal especially for the problematic propeller speeds, because the tones interference is resolved.

We should point out the parts of the simulation where the equalized signal shows higher deviation than the non-equalized signal. For example, this happens at $f_p~=36 Hz$, in Fig. \ref{fig:speed}. This is due to that the inversion of the modulation at this $f_p$ can cause interference between the signal components. 

We show this effect in Fig. {}. This is specific to this signal and will be at different speeds for different types of signal. Therefore we the system designers has to be aware that will be blind spots in the equalization process because the deconvolution/euqlization tones coincides with the signal tone spacings. And that at these spots the non-equalized signal would be better for evaluation. But in the long scale of $f_p$ we can see that these points are not frequent. 

